Cross-Domain Entity Resolution in Social Media

The challenge of associating entities across multiple domains is a key problem in social media understanding. Successful cross-domain entity resolution provides integration of information from multiple sites to create a complete picture of user and community activities, characteristics, and trends. In this work, we examine the problem of entity resolution across Twitter and Instagram using general techniques. Our methods fall into three categories: profile, content, and graph based. For the profile-based methods, we consider techniques based on approximate string matching. For content-based methods, we perform author identification. Finally, for graph-based methods, we apply novel cross-domain community detection methods and generate neighborhood-based features. The three categories of methods are applied to a large graph of users in Twitter and Instagram to understand challenges, determine performance, and understand fusion of multiple methods. Final results demonstrate an equal error rate less than 1%.

==> exp_analyze.tex <==
%
% Experimental analysis
%

\begin{itemize}
\item General commentary here about methods
\item Calculate prior for match and expected overlap between Twitter and Instagram
\item Qualitative results
\item Might not need this section ...
\end{itemize}




==> exp_sys.tex <==
%
% System performance
%

\begin{itemize}
\item Describe basic approach -- pick best distinct systems from each category 
\item Compare distinct systems
\item Commment on strengths/weaknesses of each approach ...
\end{itemize}




==> fusion.tex <==
%
% Fusion
%

The goal for fusion is to combine the similarity scores from different
features to obtain a better entity disambiguation system. Fusion was
performed using logistic regression and random forest models. The
former approach builds a linear model that predict the probability of
an outcome using the logistic distribution function; the latter
approach is an ensemble learning method that constructs a number of
decision trees and average the probabilities of an outcome from these
decision trees.

One issue arise for building the fusion models is the problem of
missing data. As mentioned earlier, for certain pair of users, the
author identification feature may be missing due to insufficient
number of words posted on their social networks. Similarly, community
(or neighborhood) feature may be missing because users are not in the
largest connected component (or they are isolates) in the aligned
graph. To address this issue, we built a separate model for each
possible subset of features.

%The goal for fusion is to combine the similarity scores from different features to obtain a better entity disambiguation system. One standard way to achieve this is to build a machine learning model. The models we choose to build are logistic regression and random forest. The former approach builds a linear model that predict the probability of an outcome using the logistic distribution function; the latter approach is an ensemble learning method that constructs a number of decision trees and average the probabilities of an outcome from these decision trees. 

%One issue arise for building the fusion models is the problem of missing data. As mentioned earlier, for certain pair of users, the author identification feature may be missing due to insufficient number of words posted on their social networks. Similarly, community (or neighborhood) feature may be missing because users are not in the largest connected component (or they are isolates) in the aligned graph. To address this issue, we employed two strategies: one is to build a separate model for each possible position of missing data and the other one is to impute the missing values. In the next section, we will explore both strategies and compare the results. 

% \begin{itemize}
% \item Discussion of approaches 
% \item Multiple fusers
% \item Imputation -- also explain why!
% \end{itemize}
% 

